CONFLLVM: A Compiler for Enforcing Data Confidentiality in Low-Level Code

We present an instrumenting compiler for enforcing data confidentiality in low-level applications (e.g. those written in C) in the presence of an active adversary. In our approach, the programmer marks secret data by writing lightweight annotations on top-level definitions in the source code. The compiler then uses a static flow analysis coupled with efficient runtime instrumentation, a custom memory layout, and custom control-flow integrity checks to prevent data leaks even in the presence of low-level attacks. We have implemented our scheme as part of the LLVM compiler. We evaluate it on the SPEC micro-benchmarks for performance, and on larger, real-world applications (including OpenLDAP, which is around 300KLoC) for programmer overhead required to restructure the application when protecting the sensitive data such as passwords. We find that performance overheads introduced by our instrumentation are moderate (average 12% on SPEC), and the programmer effort to port OpenLDAP is only about 160 LoC.

==> formal_summary.tex <==
%!TEX root=./main.tex

\section{Formal Analysis of {\protect\Verifier}}
\label{sec:formal}

\Verifier removes \cc from the Trusted Computing Base by checking that
the output binary has the required instrumentation in place. We go a
step further and formally prove that the instrumentation ensures the
security of the program. In this section, we outline important aspects
of our formalization and the main theorem statement -- detailed
formalization and proofs can be found in the accompanying technical
report.

We formalize the confidentiality of private data using the standard
notion of \emph{termination-insensitive
  noninterference}~\cite{Sabelfeld:2006:LIS:2312191.2314769}
-- for any two runs of the program that start from
\emph{low-equivalent} states (i.e. states that differ only in the
private regions), \emph{if} the two runs terminate normally then the
output states are also \emph{low-equivalent}. Intuitively, no
information from the private memory leaks to the public memory, when
the programs terminate successfully.

Let $P$ denote a program with appropriate checks in place (written as
$\vdash P$), and let $s$ denote a program state of $P$. We
formalize low-equivalence, $s_0 =_{L} s_ 1$, as $s_0$ and $s_1$ having
same  program counter, public stack contents, public heap contents,
and  register values for the registers labeled public at the current 
program counter. We denote one step of execution in the untrusted $U$
code by $s_0 \rightarrow s_1$, zero-or-more steps are denoted by the
corresponding reflexive transitive closure
$\rightarrow^*$. Finally $\bot$ is a special state modeling
unsuccessful termination (assertion failure or divergence).

We then prove the following theorem:

\begin{theorem}[Termination-insensitive noninterference]
Suppose $\vdash P$. Then, for all states $s_0$,
$s_1$ and $s_0'$ of $P$ such that $s_0 =_{L} s_1$ and
$s_0 \rightarrow^* s_0'$, then either $s_1 \rightarrow^* \bot$
or $\exists\;s_1'.\;s_1 \rightarrow^* s_1'$ and $s_1 =_{L} s_1'$.
\end{theorem}

As the reader might have guessed, the proof of this theorem is
conditioned on the trusted functions in $T$ being noninterferent
(recall that $T$ is trusted and uninstrumented). We formalize this
assumption by modeling execution of a trusted function $f$ as a
different relation $s_0 \hookrightarrow_f s_1$, with the following property:

\begin{assumption}
For all $s_0$, $s_1$, $s'_0$ such that
$s_0 =_L s_1$, if $s_0 \hookrightarrow_f s_0'$
then
$\exists\;s_1'.\;s_1 \hookrightarrow_f s_1'$ and
$s_1 =_L s_1'$.
\end{assumption}

We have proven our theorem for a core set of instructions including load,
store, binary and unary operators, direct and indirect function calls,
conditionals, and unconditional jumps. The relation $\vdash P$ for
well-instrumented $P$ is modeled as having appropriate checks before
each instruction as per our scheme. We refer the reader to the
technical report for more details.


%% Conceptually, \Verifier operates in two stages. First, it disassembles
%% a binary, constructs its control flow graph (CFG) and re-infers the
%% taints of registers at all program points. Second, it checks that the
%% taints at the beginning and end of every instruction are consistent
%% with the instruction's semantics, and that other dynamic checks
%% described in Section~\ref{sec:verifier} are correctly inserted. Here,
%% we formalize the second stage and show if a program passes those
%% checks, then the program is secure in a formal sense. We assume that
%% the disassembly and the reconstruction of the CFG from the first
%% stage, both of which use an existing tool, are correct. 

%% \begin{table}[]
%% \small
%% \begin{equation*}
%% \begin{split}
%% %% \mathit{program}  \bnfdef &
%% %%   block\kstar
%% %% \\
%% %% \mathit{block} \bnfdef &
%% %%   \mpair{\dword}{\tuple{\pc \in \values, \stmt}\kstar}
%% %% \\
%% \stmt \bnfdef &
%% %  \bcskip                                         \bnfsep 
%%   \bnfc{ldr} \of{\reg{}, exp} \ \                 \bnfsep 
%%   \bnfc{str} \of{\reg{}, exp} \                   \bnfsep 
%%   \bcjump{exp}                                    \bnfsep \\ &
%%   \beifthenelse{exp}{\bcjump{exp}}{\bcjump{exp}}  \bnfsep 
%%   \bcret{}                                        \bnfsep \\&
%%   \bccall{f}{exp^*}{\scaleto{\{\untrusted|\trusted\}}{4pt}}      \bnfsep
%%   \bicall{exp}{exp^*}                             \bnfsep 
%%   \bnfc{assert} \of{exp^*}                                                            
%% \\  
%% \mathit{exp} \bnfdef &
%%   n \in \values                         \             \bnfsep
%%   \reg{} \in \regs                      \             \bnfsep 
%%   \unaryop{exp}                         \             \bnfsep
%%   \binaryop{exp}{exp}                                 \bnfsep 
%%   \&f
%% \end{split}
%% \end{equation*}
%% \caption{Command syntax}%, here $\bitset = \{0,1\}$.}
%% \label{tbl:bil_model_syntax}
%% \end{table}

%% We model the disassembled CFG abstractly. For each function, the CFG
%% has one bit of metadata, which indicates whether the function is part
%% of the trusted code or the untrusted code (abstractly written
%% $\trusted$ and $\untrusted$, respectively). Additionally, there is a
%% 64-bit magic sequence for each function, which encodes the taints of
%% the function's arguments and its return value (see
%% Section~\ref{sec:cfi}). For trusted functions (whose code \Verifier
%% does not analyze), this is all the CFG contains. For untrusted
%% functions (whose code \Verifier does analyze), there is an additional
%% block-graph describing the code of the function. The block-graph for
%% an untrusted function $\meth$ is a tuple $\cfg_{\meth} =
%% \tuple{\cntrls_{\meth}, \edges}$ of nodes of $\meth$ and edges $\edges
%% \subseteq \cntrls \times \cntrls$. The edges represent all direct
%% control transfers. A node $\tuple{\pc, C, \seccontext, \seccontext'}
%% \in \cntrls_{\meth}$ consists of a program counter $\pc$, a single
%% command (assembly instruction) $C$, and register taints $\seccontext$
%% and $\seccontext'$ before and after the execution of $C$. $\pc$ is a
%% number, like a line number, that can be used in an indirect jump to
%% this node. $\seccontext$ and $\seccontext'$ are maps from machine
%% register ids to $\{\hseclabel, \lseclabel\}$, representing high
%% (private) and low (public) data.

%% Commands $C$ are represented in an abstract syntax shown in
%% Table~\ref{tbl:bil_model_syntax}. The auxiliary syntax of
%% \emph{expressions} consists of constants, which here can only be
%% integers that may represent ordinary data or line numbers, standard
%% binary and unary operators (ranged over by $\binaryop{}{}$ and
%% $\unaryop{}$, respectively), and the special operation $\&f$ which
%% returns the $\pc$ of the starting instruction of function $f$. We
%% assume that operations used in expressions are total, i.e.,
%% expressions never get stuck.
%% %% We prohibit pointer arithmetic
%% %% on function pointers.

%% Commands include register load $\bnfc{ldr} \of{\reg{}, exp}$ and store
%% $\bnfc{str} \of{\reg{}, exp}$ where the input $exp$ evaluates to a
%% memory location, unconditional jumps $\bcjump{exp}$, conditionals
%% $\bnfc{ifthenelse}$, direct function calls $\bccall{f}{exp^*}{\scaleto{\{\untrusted|\trusted\}}{4pt}}$, indirect
%% function calls $\bnfc{icall}$, and return $\bcret$. The subscript for $\bnfc{call}_{\scaleto{\{\untrusted|\trusted\}}{4pt}}$ 
%% denotes if the command is used to invoke an untrusted functionality or a trusted one. An additional
%% command $\bnfc{assert}$ models checks inserted by the compiler. The
%% asserted expressions must be true, else the program halts in a special
%% state $\bot$. Appendix~\ref{appendix:A} presents the operational semantic of the commands in Table~\ref{tbl:bil_model_syntax}.

%% Every CFG $\cfg$ has a designated entry function, similar to main() in
%% C programs.

%% %% In what follows,  we formalize \Verifier and show that a program satisfying requirements enforced by \Verifier is secure against illicit information leakage. 
%% %% For the theory development we consider deterministic programs written in simplified MCInst language (SMCInst) with the syntax depicted in Table~\ref{tbl:bil_model_syntax}.

%% %% A SMCInst program ($\prog \in \mathit{program}$) is a list of blocks, each consisting of a uniquely identifying label (i.e. magic strings) and a list of atomic commands. Blocks represent body of functions in the program.
%% %% %A statement can affect a program state by for example assigning the evaluation of an expression to a register or modifying flow of the execution.
%% %% %
%% %% Expressions are built using constants (i.e. integers), standard binary
%% %% and unary operators (ranged over by $\binaryop{}{}$ and $\unaryop{}$
%% %% respectively) for finite integer arithmetic\footnote{We assume that
%% %%   operations used in expressions are total.}, and function pointers
%% %% $\&f$ which are used for indirect function calls. We prohibit pointer
%% %% arithmetic on function pointers.  Commands include register load
%% %% $\bnfc{ldr} \of{\reg{}, exp}$ and store $\bnfc{str} \of{\reg{}, exp}$,
%% %% where the input $exp$ evaluates to a memory location, unconditional
%% %% jumps $\bcjump{exp}$ to change the execution flow, conditionals
%% %% $\bnfc{ifthenelse}$, direct function calls $\bnfc{call}$, indirect
%% %% function calls $\bnfc{icall}$ and return $\bcret$. We also provide
%% %% $\bnfc{assert}$; the asserted expression must be true, else the
%% %% program halts with $\bot$.
%% %Note that $\bnfc{assert}$ is used to check conditions which must hold only at runtime.


%% \noindent{\textbf{Dynamic semantics.}}
%% A program/CFG $\cfg$ can be evaluated in a context of a data memory
%% $\mem:\!\values\!\to\!\values$, a register state
%% $\regstate:\!\regs\!\to\!\values$ and a program counter $\pc$ which
%% points to a node in the program's CFG. The memory $\mem$ is actually a
%% union of two maps $\mem_{\lseclabel}$ and $\mem_{\hseclabel}$ over
%% disjoint domains, representing the low and the high regions of memory
%% of our scheme.
%% %
%% %% Each store, i.e. a memory location or a register, are assigned a
%% %% security type $\seclabel \in \seclabelstate$, and $(\seclabelstate,
%% %% \sqcup, \sqsubseteq)$ is a lattice of security levels.  We assume a
%% %% two-level security lattice consisting of $\hseclabel$ for
%% %% confidential stores and $\lseclabel$ for stores containing public
%% %% information, with $\lseclabel \sqsubseteq \hseclabel$.  Moreover,
%% %% $\seccontext$ is the \textit{typing context}, and it consists of
%% %% hypotheses of the form $x : \seclabel$, one for each store.
%% %% Security level of memory locations is fixed and assigned
%% %% statically, but registers taint is determined dynamically.
%% %This makes the analysis \textit{flow sensitive}.
%% %
%% Given a fixed $\cfg$, a \textit{configuration} $\config$ of $\cfg$ is
%% a record $\tuple{\mem, \regstate,  [\stack_{\hseclabel}:\stack_{\lseclabel}], \pc}$ of the entire
%% state---the memory, register state, stack, and the program counter. We
%% make a distinction between high ($\stack_{\hseclabel}$) and low
%% ($\stack_{\lseclabel}$) stacks. We write $\elem{\tuple{.}}{i}$ to
%% project a tuple to its $i$th component. Thus, if $\config =
%% \tuple{\mem, \regstate, [\stack_{\hseclabel}:\stack_{\lseclabel}], \pc}$,
%% then $\config.\pc = \pc$. We call a configuration $\config$ initial
%% (final) if $\config.\pc$ is the first (last) node of the entry
%% function of $\cfg$.

%% %\aseem{what is the grammar for stack? briefly mention?}

%% Next, we define the dynamic semantics of a program as a transition
%% relation $\config \to \config'$. The rules of this relation are the
%% expected ones, so we omit them here. We only note that calls to
%% trusted functions, whose code is not modeled in the CFG, are
%% represented via an external relation $\config \hookrightarrow_{\meth}
%% \config'$ that models the entire execution of the trusted function
%% $\meth$ and its effects on the configuration. The special transition
%% $\config \to \bot$ means that $\config.\pc$ contains an
%% $\bnfc{assert}$ command, one of whose arguments evaluates to
%% false. $\bot$ does not transition any further. 
%% Furthermore, the transition $\config \to \confgiAdversary$ is used to model adversarial behaviour, for example,
%% when the  target of $\bnfc{icall}$ is not in the CFG.
%% $\confgiAdversary$ resembles a configuration where memory locations are loaded with random values.

%% %% The CFG is defined as a disjoint union of \textit{block-graphs}, one for each function in the program.
%% %%  A block-graph for a function $\meth$  is a tuple
%% %% $\cfg_{\meth} = \tuple{\cntrls_{\meth}, \edges}$ of control nodes 
%% %% of $\meth$ and edges $\edges \subseteq \cntrls \times \cntrls$. A node $\tuple{\pc, C, \seccontext, \seccontext'} \in \cntrls_{\meth}$ consists of program counter, (single) command, and  typing contexts before and after executing
%% %% the command $C$.

%% %% We define $\mathit{pred}$ ($\mathit{succ}$) as the function which
%% %% operates on the CFG and returns the predecessors (successors) of the
%% %% input node, $\mathit{pred}, \mathit{succ}: \cfgs times \vals \to
%% %% \cntrls^*$. And, $\elem{\tuple{.}}{i}$ is used to project a tuple to
%% %% its $i$th component.
%% %

%% \noindent{\textbf{{Security Analysis.}}
%% We formalize the checks that \Verifier makes via the judgment $\cfg
%% \vdash\seccontext \{pc\} \seccontext'$, which means that the command
%% in the node labeled $\pc$ in the CFG $\cfg$ is consistent with the
%% beginning and ending taints $\seccontext$ and $\seccontext'$, and that
%% the checks from Section~\ref{sec:verifier} corresponding to this
%% command are satisfied. Selected rules for this judgment are shown in
%% Figure~\ref{symsem}. The function $\mathit{pred}(\cfg, \pc)$ returns
%% the predecessors of the node labeled $\pc$ in $\cfg$. For $\seclabel
%% \in \{\lseclabel, \hseclabel\}$, $\bnfc{assert}(e \in
%% \preimg(\mem_{\seclabel}))$ represents the dynamic check that $e$
%% evaluates to an address in the domain of $\mem_{\seclabel}$, and the
%% auxiliary judgment $\seccontext \vdash e : \seclabel$ means that the
%% expression $e$ depends only on values with secrecy $\seclabel$ or
%% lower.


%% \begin{figure}
%% \centering
%% {\small
%% \begin{tabular}{c}

%% \begin{math}
%% \prooftree
%% \begin{array}{c}
%%  C\!=\!\bnfc{ldr}(\reg{},e) \\  \forall\ \cntrl \!\in\!\pred{\cfg}{\pc}.\ \elem{\cntrl}{C}\!=\!\bnfc{assert}(e \in \preimg(\mem_{\seclabel_e})) 
%% \end{array}
%% \justifies
%% \begin{array}{c}
%%  \cfg \vdash \seccontext \{\pc\} \seccontext[reg \mapsto \seclabel_e]
%% \end{array}
%% \endprooftree  
%% \end{math} \\[15pt]

%% \begin{math}
%% \prooftree
%% \begin{array}{c}
%%  C\!=\!\bnfc{str}(\reg{},e)\ \ \ \  \seccontext \vdash \reg{}: \seclabel_r \ \ \ \ \seclabel_r  \sqsubseteq \seclabel_{e}\\
%%  \forall \cntrl\!\in\!\pred{\cfg}{\pc}.\ \elem{\cntrl}{C}\!=\!\bnfc{assert}(e\!\in\!\preimg(\mem_{\seclabel_{e}}))
%% \end{array}
%% \justifies
%% \begin{array}{l}
%%  \cfg \vdash \seccontext \{\pc\} \seccontext
%% \end{array}
%% \endprooftree  
%% \end{math}
%% \\[15pt]

%% \begin{math}
%% \prooftree
%% \begin{array}{l}
%% C = \bnfc{goto}\of{e}\ \ \ \ \seccontext \vdash e:\seclabel_e\ \ \ \ \seclabel_e \sqsubseteq \lseclabel
%% \end{array}
%% \justifies
%% \begin{array}{l}
%% \cfg \vdash \seccontext\ \{\pc\}\ \seccontext
%% \end{array}
%% \endprooftree 
%% \end{math}\\[15pt]

%% \begin{math}
%% \prooftree
%% \begin{array}{c}
%% C = \beifthenelse{e}{\bcjump{e_1}}{\bcjump{e_2}} \ \  \seccontext \vdash e: \seclabel_e \ \ \ \seclabel_e \sqsubseteq \lseclabel
%% \end{array}
%% \justifies
%% \begin{array}{l}
%% \cfg \vdash \seccontext\ \{\pc\}\ \seccontext
%% \end{array}
%% \endprooftree 
%% \end{math}

%% \end{tabular}
%% }
%% \caption{Selected type rules. $C$ is the command in the CFG node
%%   pointed to by $\pc$. }
%% \label{symsem}
%% \end{figure}

%% The rules are mostly self-explanatory. The first rule, which is for
%% the command $\bnfc{ldr}(\mathit{reg}, e)$, says that if $\mathit{reg}$
%% has taint $\seclabel_e$ after the command, then on all paths leading
%% to this command, there must be a check that whatever $e$ evaluates to
%% is actually pointing into $\mem_{\seclabel_e}$. The second rule, for
%% $\bnfc{str}$, is similar. In the rules for indirect branching, we
%% insist that the addresses of the branch targets have the taint
%% $\lseclabel$. Overall, our type system's design is inspired by the
%% flow-sensitive information flow type system of Hunt and
%% Sands~\cite{Hunt:2006:FST:1111037.1111045}. However, the runtime
%% checks are new to our system. (The appendix has all the rules of the
%% type system.)

%% We say that a CFG $\cfg$ is well-typed (passes \Verifier's checks),
%% written $\vdash \cfg$, when two conditions hold for all nodes $\cntrl$
%% in (untrusted functions in) $\cfg$: 1) The node (locally) satisfies
%% the type system. Formally, $\cfg \vdash \cntrl.\seccontext \;
%% \{\cntrl.\pc\}\; \cntrl.\seccontext'$, and 2) The ending taint of the
%% node is consistent with the beginning taints of all its
%% successors. Formally, for all nodes $\cntrl' \in \mathit{succ}(\cfg,
%% \cntrl.\pc)$, $\cntrl.\seccontext' \sqsubseteq \cntrl'.\seccontext$,
%% where $\mathit{succ}(\cfg, \pc)$ returns the successors of the node
%% labeled $\pc$ in $\cfg$. We emphasize again that only untrusted
%% functions are checked.

%% \noindent{\textbf{Security theorem.}}
%% The above checks are sufficient to prove our key theorem: If a program
%% passes \Verifier, then assuming that its trusted functions don't leak
%% private data, the whole program does not leak private data,
%% end-to-end. We formalize non-leakage of private data as the standard
%% information flow property called \emph{termination-insensitive
%%   noninterference}. Roughly, this property requires a notion of low
%% equivalence of program configurations (of the same CFG $\cfg$),
%% written $\config \leqv \config'$, which allows memories of $\config$
%% and $\config'$ to differ only in the private region.  A program is
%% noninterfering if it \emph{preserves} $\leqv$ for any two runs, except
%% when one program halts safely (e.g., on a failed
%% assertion). Intuitively, noninterference means that no information
%% from the private part of the initial memory can leak into the public
%% part of the final memory.

%% For our model, we define $\config \leqv \config'$ to hold if: (i)
%% $\config$ and $\config'$ point to the same command, i.e., $\config.\pc
%% = \config'.\pc$, (ii) the contents of their low-stacks are equal,
%% $\config.\stack_{\lseclabel} = \config'.\stack_{\lseclabel}$, (iii)
%% for all low memory addresses $m \in \mem_{\lseclabel}$,
%% $\config.\mem(m) = \config'.\mem(m)$, (iv) for all registers $r$ such
%% that $\cfg(\config.\pc).\seccontext(r) = \lseclabel$,
%% $\config.\regstate(r) = \config'.\regstate(r)$.

%% %% We define the mode of a configuration $\mode(\config)$ as the label
%% %% $\trusted$ or $\untrusted$ of the function in which $\config.\pc$
%% %% lies. We write $\config \to_{\tau} \config'$ when $\config \to
%% %% \config'$ and $\mode(\config) = \tau$.

%% The assumption that trusted code does not leak private data is
%% formalized as follows.

%% \begin{assumption}
%% For all $\config_0$, $\config_1$, $\config'_0$ such that $\config_0
%% \leqv \config_1$, if $\config_0 \hookrightarrow_{\meth} \config'_0$
%% then $\exists \config'_1. \ \config_1 \hookrightarrow_{\meth}
%% \config'_1$ and $\config'_0 \leqv \config'_1$.
%% \end{assumption}

%% Under this assumption on the trusted code, we can show the
%% noninterference or security theorem. 
%% A necessary condition to show noninterference, however, is to ensure that no well-typed program can reach an ill-formed configuration.

%% \begin{lemma}\label{lem:noAdversarialConfig}
%%  Suppose $\vdash \cfg$, for all configurations $\config$ of $\cfg$  it holds that $\config \nrightarrow^* \confgiAdversary$.
%% \end{lemma}

%% Lemma~\ref{lem:noAdversarialConfig} rules out possible nondeterminism caused by adversarial behaviour and allows to formalize the security theorem as follows.

%% \begin{theorem}[Termination-insensitive noninterference]
%% Suppose $\vdash \cfg$. Then, for all configurations $\config_0$,
%% $\config_0'$ and $\config_1$ of $\cfg$ such that $\config_0 \leqv
%% \config_1$ and $\config_0 \to^* \config'_0$, then either $\config_1
%% \to^* \bot$ or $\exists \config'_1.\ \config_1 \to^* \config'_1$ and
%% $\config'_0 \leqv \config'_1$.
%% \end{theorem}

%% When $\config_0$ and $\config_0'$ are initial and final
%% configurations, respectively, then $\config_1$ and $\config_1'$ must
%% also be initial and final configurations, so the theorem guarantees
%% freedom from data leaks, end-to-end (modulo assertion check failures).



%% %% In words, this theorem says that transitions from a configuration can
%% %% be simulated from any other configuration related by $\leqv$,
%% %% eventually ending in $\leqv$ configurations (modulo the possibility of
%% %% assertion failures in either run).

%% %% %
%% %% Our typing judgments have the form $\cfg \vdash\seccontext \{pc\} \seccontext'$, where $\cfg$ is the CFG.
%% %% Intuitively, the judgment expresses that the security level of stores are determined by $\seccontext$ before executing the command pointed to by $\pc$, and $\seccontext'$
%% %% contains the security level of stores afterward.
%% %% Moreover, the judgment $\seccontext \vdash e : \seclabel$ is used to determine that the security level of the expression $e$ is $\seclabel$, and it is defined as the join of security
%% %% level of stores in $e$. 
%% %% % Formally: $\seccontext \vdash e : \seclabel$, where $\seclabel = \bigsqcup_{x \in \mathit{st}(e)} \seccontext(x)$, and $\mathit{st}$ returns the set of memory locations 
%% %% % and registers used in $e$. We over-load the notation to handle tuple of expressions to simplify the type checking rules. 

%% %% Our type system, in addition to enforcing static checks, ensures that the program is properly annotated with runtime checks, which are essential, e.g., to prevent leaks through pointers.\todo[inline]{is this right? I read this in the introduction.}
%% %% We use the $\bnfc{assert}$ command to summarize the conditions which must hold at runtime. 
%% %% For example, $\bnfc{assert}(e \in \preimg(\mem_{\seclabel}))$, in the $\bnfc{ldr}$ rule, checks if the expression $e$ is in the domain of the memory partition with statically inferred security type ${\seclabel}$.

%% % We say the control-flow graph $\cfg$ is well-typed, and write $\vdash\!\cfg$, if for every $\cfg_{\meth} = \tuple{\cntrls_{\meth}, \edges}$ in $\cfg$ :
%% % (i) $\forall \cntrl \in \cntrls_{\meth}.\ \ \vdash \cntrl.\seccontext\ \{\cntrl.\pc\}\ \cntrl.\seccontext'$ and 
%% % (ii) $\forall \cntrl, \cntrl' \in \cntrls_{\meth}.\ \cntrl' \in \suc{\cfg}{\cntrl.\pc} \text{ and }  \cntrl.\seccontext' = \cntrl'.\seccontext$.
%% % That is the typing context of consecutive nodes are properly connected.

%% %% We say the control-flow graph $\cfg$ is well-typed, and write $\vdash\!\cfg$, if for every $\cfg_{\meth} = \tuple{\cntrls_{\meth}, \edges}$ in $\cfg$ :
%% %% (i) the typing contexts of control nodes in $\cfg_{\meth}$ are consistent with the type rules (i.e., $\forall \cntrl \in \cntrls_{\meth}.\ \ \vdash \cntrl.\seccontext\ \{\cntrl.\pc\}\ \cntrl.\seccontext'$), and 
%% %% (ii) the typing contexts of consecutive nodes are properly connected (i.e., $\forall \cntrl, \cntrl' \in \cntrls_{\meth}.\ \cntrl' \in \suc{\cfg}{\cntrl.\pc} \text{ and }  \cntrl.\seccontext' = \cntrl'.\seccontext$).

%% %% We formulate the system security as a \textit{noninterference} property and show that a program which is compliant with typing constraints is noninterfering.
%% %% The program in our analysis either executes in untrusted context $\untrusted$ or invokes a trusted functionality $\trusted$.
%% %% We define the behaviour of the system as a labeled transition system $\to_{\tau} \subseteq \configs \times \configs \cup \{\bot\}$, where $\tau \in \{\trusted, \untrusted\}$,
%% %% and if $\config \to_{\tau} \config'$ then $\mode({\config}) = \tau$. Each transition represents execution of a command from the program CFG.
%% %%  A transition may fail if the condition of an $\bnfc{assert}$ statement does not hold, which can only happen in the untrusted context.
%% %% We also introduce a weak transition relation which is used to hide trusted transitions;
%% %% i.e., $\config \weaktrs \config'$ such that $\mode(\config') = \untrusted$. This relation behaves as a normal transition if $\mode({\config}) = \untrusted$. 
%% %% However, if $\mode({\config}) = \trusted$ then the transition relation atomically transforms the system state and yields a configuration in the untrusted context.
%% %if there exists $\config_0\!\to\!\dots\!\to\!\config_n$ such that $\mode(\config_n) = \untrusted$ and $\mode(\config_j) \neq \untrusted$ for $0 < j < n$.% An example of such transitions is illustrated in Figure~\ref{wktrans}.


%% %% Noninterference is a two-state property and requires reasoning about two runs of the program. 
%% %% We say a program is noninterfering if any transitions from low-equivalent configurations, when both the program runs succeed, end in configurations which are in the low-equivalence relation.

%% %% \begin{theorem}
%% %%  For all configurations $\config_0$ and $\config_1$ such that $\vdash\!\cfg\footnotemark$ and $\config_0 \leqv \config_1$ and $\config_0 \weaktrs \config'_0$, if $\config_1 \not{\weaktrs} \bot$ then
%% %%  $\exists \config'_1.\ \config_1 \weaktrs \config'_1$ and  $\config'_0 \leqv \config'_1$. 
%% %% \end{theorem}
%% %% \footnotetext{Since the CFG is fixed, in the sequel we skip writing configuration prefix to simplify presentation.}

%% %% In our analysis trusted functionalities  are noninterfering if the initial states of two runs after switching to the trusted context are in the relation $\tentry(\config_0, \config_1)$. 
%% %% This predicate ensures that $\config_0$ and $\config_1$ are reachable immediately after switching to the trusted context and that, in a very simple setting, $\config_0$ and $\config_1$ are in the low-equivalent relation.
%% %% However, the predicate $\tentry$ may express more complex conditions depending on the type of invoked trusted functionalities.
%% %% %\todo[inline]{Adding the condition which we discussed in the meeting.}.

%% %% \begin{assumption}
%% %% For all  $\config_0$, $\config_1$, $\config'_0$ such that $\vdash\!\cfg$
%% %% and $\mode(\config_0) = \mode(\config_1) = \trusted$ and $\tentry(\config_0, \config_1)$, If $\config_0 \weaktrs \config'_0$ then $\exists \config'_1. \ \config_1 \weaktrs \config'_1$ and
%% %% $\config'_0 \leqv \config'_1$.
%% %% \end{assumption}

%% %% Then to show that the system is secure, we need to prove that the untrusted transitions are noninterfering, and context switching yields states that are in the relation $\tentry$.
%% %% \begin{lemma}\label{lem:userConfidentiality}
%% %%  For all $\config_0$ and $\config_1$ such that $\vdash\!\cfg$ and $\config_0 \leqv \config_1$ and $\config_0 \uto \config'_0$ 
%% %%  (i) if  $\config_1 \not{\uto} \bot$ then $\exists \config'_1.\ \config_1 \uto \config'_1$ and $\config'_0 \leqv \config'_1$, and 
%% %%  (ii) if $\mode(\config'_0) = \trusted$ and $\config_1 \not{\uto} \bot$ then
%% %%  $\exists \config'_1.\ \config_1 \uto \config'_1$ and $\mode(\config'_1) = \trusted$ and  $\tentry (\config'_0, \config'_1)$.
%% %% \end{lemma}
%% %% %
%% %% Central to proving Lemma~\ref{lem:userConfidentiality} is to showing that at each step untrusted transitions in two runs execute the same instructions, or in another words two runs will follow the same path in the CFG. 
%% %% Proof of this last property depends on the two characteristics of our system, namely (i) the target of unconditional jumps are always low and (ii) conditional expression in $\bnfc{ifthenelse}$ cannot be high.









==> ms.tex <==
\input{paper-sigplan}


